jazznet: A Dataset of Fundamental Piano Patterns for Music Audio Machine Learning Research

This paper introduces the jazznet Dataset, a dataset of fundamental jazz piano music patterns for developing machine learning (ML) algorithms in music information retrieval (MIR). The dataset contains 162520 labeled piano patterns, including chords, arpeggios, scales, and chord progressions with their inversions, resulting in more than 26k hours of audio and a total size of 95GB. The paper explains the dataset's composition, creation, and generation, and presents an open-source Pattern Generator using a method called Distance-Based Pattern Structures (DBPS), which allows researchers to easily generate new piano patterns simply by defining the distances between pitches within the musical patterns. We demonstrate that the dataset can help researchers benchmark new models for challenging MIR tasks, using a convolutional recurrent neural network (CRNN) and a deep convolutional neural network. The dataset and code are available via: https://github.com/tosiron/jazznet.

==> classLevelResults.tex <==
\begin{table}[]
\caption{Average precision on the \textit{large} subset}
\label{tab:classResults}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l||l}
\hline
Class      & CRNN & DCNN & Person1 (\%) & Person2 (\%) \\ \hline
\textbf{Chords} & 100 & 28 & 83 (for dim7-chord)  & 55  & 40         \\ \hline
\textbf{Arpeggios} & 95 & 16 & 65 (for tritone-arpeggio) & 70 & 90 \\ \hline
\textbf{Scales} & 94 &  10  & 56 (for pentatonic) & 55 & 100    \\ \hline
\textbf{Progressions} & 100  & 67 & 99 (for I-IV7-iii-VI7) & 70 & 71\\ \hline
\end{tabular}

\end{table}

==> progGeneration.tex <==
\begin{algorithm}[t]
\small
\DontPrintSemicolon
\caption{Chord progression generation via \textit{distance-based pattern structures}}\label{alg:progGeneration}
\KwIn{progression = [$p_0$,$p_1$,...,$p_n$], where $p_i$ is a Roman numeral $I/i to VIII/viii$;}
\KwOut{Chord progressions in all keys}
\ForEach{MIDI\_pitch \textbf{in} range(24, 109)}{
$note_0 \gets$ MIDI\_pitch\;

$time \gets time$ \textit{\#current time}

\For{i \textbf{in} range(0, len(distance) - 1)}{
$note_{i+1} \gets note_i + distance[i]$\;
\If{type == "arpeggio" or "scale"}{
$time \gets time+1$
}
}
}
\end{algorithm}

==> taxBackup.tex <==
\tikzset{
  basic/.style  = {draw, text width=3cm, drop shadow, font=\sffamily, rectangle},
  root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white},
  level-2/.style = {basic, rounded corners=6pt, thin,align=center, fill=white, text width=3cm},
  level-3/.style = {basic, thin, align=center, fill=white, text width=1.8cm, text height=0.2cm}
}

\begin{figure}
\small
    \centering
\begin{tikzpicture}[
  level 1/.style={sibling distance=12em, level distance=3em},
%   {edge from parent fork down},
  edge from parent/.style={->,solid,black,thick,sloped,draw}, 
  edge from parent path={(\tikzparentnode.south) -- (\tikzchildnode.north)},
  >=latex, node distance=0.4cm, edge from parent fork down]

% root of the the initial tree, level 1
\node[root] {\textbf{jazzNet}}
% The first level, as children of the initial tree
  child {node[level-2] (c1) {\textbf{Chords}}}
  child {node[level-2] (c2) {\textbf{Arpeggios}}}
  child {node[level-2] (c3) {\textbf{Scales}}}
  child {node[level-2] (c4) {\textbf{Progressions}}};

% The second level, relatively positioned nodes
\begin{scope}[every node/.style={level-3}]
\node [below of = c1, xshift=10pt] (c11) {min2};
\node [below of = c11] (c12) {maj2};
\node [below of = c12] (c13) {min3};
\node [below of = c13] (c14) {maj3};
\node [below of = c14] (c15) {perf4};
\node [below of = c15] (c16) {tritone};
\node [below of = c16] (c17) {perf5};
\node [below of = c17] (c18) {min6};
\node [below of = c18] (c19) {maj6};
\node [below of = c19] (c110) {aug6};
\node [below of = c110] (c111) {maj7-2};
\node [below of = c111] (c112) {octave};
\node [below of = c112] (c113) {aug};
\node [below of = c113] (c114) {dim};
\node [below of = c114] (c115) {dim7};
\node [below of = c115] (c116) {maj};
\node [below of = c116] (c117) {maj7};
\node [below of = c117] (c118) {min};
\node [below of = c118] (c119) {min7};
\node [below of = c119] (c120) {seventh};
\node [below of = c120] (c121) {sixth};
\node [below of = c121] (c122) {sus2};
\node [below of = c122] (c123) {sus4};

\node [below of = c2, xshift=10pt] (c21) {min2};
\node [below of = c21] (c22) {maj2};
\node [below of = c22] (c23) {min3};
\node [below of = c23] (c24) {maj3};
\node [below of = c24] (c25) {perf4};
\node [below of = c25] (c26) {tritone};
\node [below of = c26] (c27) {perf5};
\node [below of = c27] (c28) {min6};
\node [below of = c28] (c29) {maj6};
\node [below of = c29] (c210) {aug6};
\node [below of = c210] (c211) {maj7-2};
\node [below of = c211] (c212) {octave};
\node [below of = c212] (c213) {aug};
\node [below of = c213] (c214) {dim};
\node [below of = c214] (c215) {dim7};
\node [below of = c215] (c216) {maj};
\node [below of = c216] (c217) {maj7};
\node [below of = c217] (c218) {min};
\node [below of = c218] (c219) {min7};
\node [below of = c219] (c220) {seventh};
\node [below of = c220] (c221) {sixth};
\node [below of = c221] (c222) {sus2};
\node [below of = c222] (c223) {sus4};

\node [below of = c3, xshift=10pt] (c31) {aeolian};
\node [below of = c31] (c32) {dorian};
\node [below of = c32] (c33) {ionian};
\node [below of = c33] (c34) {locrian};
\node [below of = c34] (c35) {lydian};
\node [below of = c35] (c36) {mixolydian};
\node [below of = c36] (c37) {phrygian};
\node [below of = c37] (c38) {pentatonic};

\node [below of = c4, xshift=10pt] (c41) {ii-V-I};
\node [below of = c41] (c42) {ii-V-i};
\node [below of = c42] (c43) {ii-triV-I};
\node [below of = c43] (c44) {I-VI-ii-V};
\node [below of = c44] (c45) {i-vi-ii-V};
\node [below of = c45] (c46) {iii-IV-ii-V};
\node [below of = c46] (c47) {I-i$\sharp$-ii-V};
\node [below of = c47] (c48) {I-IV7-iii-VI7};
\node [below of = c48] (c49) {ii$\sharp$-V$\sharp$-ii-V};
\end{scope}

% lines from each level 1 node to every one of its "children"
\foreach \value in {1,...,23}
  \draw[->] (c1.195) |- (c1\value.west);
  
\foreach \value in {1,...,23}
  \draw[->] (c2.195) |- (c2\value.west);
  
\foreach \value in {1,...,8}
  \draw[->] (c3.195) |- (c3\value.west);
  
\foreach \value in {1,...,9}
  \draw[->] (c4.195) |- (c4\value.west);

\end{tikzpicture}
    \caption{High-level taxonomy of the jazzNet Dataset.}
    \label{fig:taxonomy}
\end{figure}
